Learning to Localize Objects Improves Spatial Reasoning in Visual-LLMs

Integration of Large Language Models (LLMs) into visual domain tasks, resulting in visual-LLMs (V-LLMs), has enabled exceptional performance in vision-language tasks, particularly for visual question answering (VQA). However, existing V-LLMs (e.g. BLIP-2, LLaVA) demonstrate weak spatial reasoning and localization awareness. Despite generating highly descriptive and elaborate textual answers, these models fail at simple tasks like distinguishing a left vs right location. In this work, we explore how image-space coordinate based instruction fine-tuning objectives could inject spatial awareness into V-LLMs. We discover optimal coordinate representations, data-efficient instruction fine-tuning objectives, and pseudo-data generation strategies that lead to improved spatial awareness in V-LLMs. Additionally, our resulting model improves VQA across image and video domains, reduces undesired hallucination, and generates better contextual object descriptions. Experiments across 5 vision-language tasks involving 14 different datasets establish the clear performance improvements achieved by our proposed framework.

==> figures/keyword_frequency.tex <==
\begin{table}[]
\begin{tabular}{lllll}
Template & left & right & left (\%) & right (\%) \\
x        & 1624 & 5006  & 0.37      & 1.13       \\
x side   & 75   & 110   &           &            \\
the x    & 240  & 1473  &           &            \\
x of     & 33   & 183   &           &           
\end{tabular}
\end{table}
